Guaranteed Conformance of Neurosymbolic Models to Natural Constraints

Deep neural networks have emerged as the workhorse for a large section of robotics and control applications, especially as models for dynamical systems. Such data-driven models are in turn used for designing and verifying autonomous systems. They are particularly useful in modeling medical systems where data can be leveraged to individualize treatment. In safety-critical applications, it is important that the data-driven model is conformant to established knowledge from the natural sciences. Such knowledge is often available or can often be distilled into a (possibly black-box) model. For instance, an F1 racing car should conform to Newton's laws (which are encoded within a unicycle model). In this light, we consider the following problem - given a model $M$ and a state transition dataset, we wish to best approximate the system model while being a bounded distance away from $M$. We propose a method to guarantee this conformance. Our first step is to distill the dataset into a few representative samples called memories, using the idea of a growing neural gas. Next, using these memories we partition the state space into disjoint subsets and compute bounds that should be respected by the neural network in each subset. This serves as a symbolic wrapper for guaranteed conformance. We argue theoretically that this only leads to a bounded increase in approximation error; which can be controlled by increasing the number of memories. We experimentally show that on three case studies (Car Model, Drones, and Artificial Pancreas), our constrained neurosymbolic models conform to specified models (each encoding various constraints) with order-of-magnitude improvements compared to the augmented Lagrangian and vanilla training methods. Our code can be found at: https://github.com/kaustubhsridhar/Constrained_Models

==> sections/wrapfigure.tex <==
\begin{wrapfigure}{r}{0.6\textwidth}
\begin{center}
\includegraphics[width=6cm, height = 4cm]{Figures/illustrative_figure.png}
\end{center}
\vspace{-8mm}
 \caption{\footnotesize The $\mathcal{X}-\mathcal{Y}$ plane is partitioned into polyhedrons using a Neural-Gas. For inputs from each polyhedron we generate sound under-approximations of the model $M$'s output. 
 % Next, we constrain the estimated function $f_\theta$ to respect these interval constraints.
 Next, we learn the function $f_{\theta}$ that is constrained by construction to respect these interval constraints.
 }
 \vspace{-8mm}
\label{fig:idea}
% \vspace{-2mm}
\end{wrapfigure}

==> tables/bicycle.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[H]
\centering
\begin{tabular}{cc|ccccc}
\hline
\multicolumn{2}{c|}{Method}                                                                                                              & \begin{tabular}[c]{@{}c@{}}Avg. \\ Approx. \\ Loss\end{tabular} & \begin{tabular}[c]{@{}c@{}}Avg. \\ CL\end{tabular} & \begin{tabular}[c]{@{}c@{}}Max. \\ CL\end{tabular} & \begin{tabular}[c]{@{}c@{}}Avg. \\ Adv.\\ CL\end{tabular} & \begin{tabular}[c]{@{}c@{}}Max. \\ Adv. \\ CL\end{tabular} \\ \hline
\multicolumn{2}{c|}{Vanilla}                                                                                                             & 0.002                                                           & 0.162                                              & 0.211                                              & 0.171                                                     & 0.691                                                      \\
\multicolumn{2}{c|}{Lagrangian}                                                                                                          &                                                                 &                                                    &                                                    &                                                           &                                                            \\
\multirow{5}{*}{\begin{tabular}[c]{@{}c@{}}Constrained\\ (Ours) with \\ num\_memories=\end{tabular}}              & 1k                   & 0.120                                                           & 0.125                                              & 0.150                                              & 0.126                                                     & 0.640                                                      \\
                                                                                                                  & 2k                   & 0.110                                                           & 0.091                                              & 0.114                                              & 0.091                                                     & 0.536                                                      \\
                                                                                                                  & 4k                   & 0.105                                                           & 0.063                                              & 0.075                                              & 0.062                                                     & 0.381                                                      \\
                                                                                                                  & 5k                   & 0.100                                                           & 0.055                                              & \underline{0.070}                                              & 0.055                                                     & \underline{0.317}                                                      \\
                                                                                                                  & 10k                  & 0.100                                                           & 0.032                                              & \textbf{0.046}                                              & 0.032                                                     & \textbf{0.226}                                                      \\ \hline
\multicolumn{2}{c|}{Self-Sup. Lagrangian}                                                                                                &                                                                 &                                                    &                                                    &                                                           &                                                            \\
\multirow{4}{*}{\begin{tabular}[c]{@{}c@{}}Self-Sup. \\ Constrained\\ (Ours) with \\ num\_memories=\end{tabular}} & \multirow{2}{*}{5k}  & \multirow{2}{*}{}                                               & \multirow{2}{*}{}                                  & \multirow{2}{*}{}                                  & \multirow{2}{*}{}                                         & \multirow{2}{*}{}                                          \\
                                                                                                                  &                      &                                                                 &                                                    &                                                    &                                                           &                                                            \\
                                                                                                                  & \multirow{2}{*}{10k} & \multirow{2}{*}{}                                               & \multirow{2}{*}{}                                  & \multirow{2}{*}{}                                  & \multirow{2}{*}{}                                         & \multirow{2}{*}{}                                          \\
                                                                                                                  &                      &                                                                 &                                                    &                                                    &                                                           &                                                            \\ \hline
\end{tabular}
\caption{With comparably small values of approximation loss, constrained neural network training increasingly outperform Lagrangian method with increasing number of memories. (Total datapoints: $>40$k)}
\end{table}

==> tables/quadrotors.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[H]
\centering
\begin{tabular}{cc|ccccc}
\hline
\multicolumn{2}{c|}{Method}                                                                                                              & \begin{tabular}[c]{@{}c@{}}Avg. \\ Approx. \\ Loss\end{tabular} & \begin{tabular}[c]{@{}c@{}}Avg. \\ CL\end{tabular} & \begin{tabular}[c]{@{}c@{}}Max. \\ CL\end{tabular} & \begin{tabular}[c]{@{}c@{}}Avg. \\ Adv.\\ CL\end{tabular} & \begin{tabular}[c]{@{}c@{}}Max. \\ Adv. \\ CL\end{tabular} \\ \hline
\multicolumn{2}{c|}{Vanilla}                                                                                                             & 0.002                                                           & 0.119                                              & 0.136                                              & 0.169                                                     & 0.626                                                      \\
\multicolumn{2}{c|}{Lagrangian}                                                                                                          & 0.032                                                           & 0.031                                              & 0.035                                              & 0.048                                                     & 0.382                                                      \\
\multirow{5}{*}{\begin{tabular}[c]{@{}c@{}}Constrained\\ (Ours) with \\ num\_memories=\end{tabular}}              & 1k                   & 0.086                                                           & 0.013                                              & 0.018                                              & 0.014                                                     & 0.382                                                      \\
                                                                                                                  & 2k                   & 0.094                                                           & 0.008                                              & 0.011                                              & 0.009                                                     & 0.320                                                      \\
                                                                                                                  & 4k                   & 0.098                                                           & 0.005                                              & 0.007                                              & 0.005                                                     & 0.151                                                      \\
                                                                                                                  & 5k                   & 0.102                                                           & 0.004                                              & \underline{0.006}                                              & 0.005                                                     & \underline{0.180}                                                      \\
                                                                                                                  & 10k                  & 0.109                                                           & 0.002                                              & \textbf{0.004}                                              & 0.003                                                     & \textbf{0.061}                                                      \\ \hline
\multicolumn{2}{c|}{Self-Sup. Lagrangian}                                                                                                &                                                                 &                                                    &                                                    &                                                           &                                                            \\
\multirow{4}{*}{\begin{tabular}[c]{@{}c@{}}Self-Sup. \\ Constrained\\ (Ours) with \\ num\_memories=\end{tabular}} & \multirow{2}{*}{5k}  & \multirow{2}{*}{}                                               & \multirow{2}{*}{}                                  & \multirow{2}{*}{}                                  & \multirow{2}{*}{}                                         & \multirow{2}{*}{}                                          \\
                                                                                                                  &                      &                                                                 &                                                    &                                                    &                                                           &                                                            \\
                                                                                                                  & \multirow{2}{*}{10k} & \multirow{2}{*}{}                                               & \multirow{2}{*}{}                                  & \multirow{2}{*}{}                                  & \multirow{2}{*}{}                                         & \multirow{2}{*}{}                                          \\
                                                                                                                  &                      &                                                                 &                                                    &                                                    &                                                           &                                                            \\ \hline
\end{tabular}
\caption{With comparably small values of approximation loss, constrained neural network training increasingly outperform Lagrangian method with increasing number of memories. (Total datapoints: $>57$k)}
\end{table}
